Search for a Fermiophobic Higgs Boson Decaying into Diphotons in p p-bar Collisions at sqrt{s} = 1.96 TeV

A search for a narrow diphoton mass resonance is presented based on data from 3.0 fb^{-1} of integrated luminosity from p-bar p collisions at sqrt{s} = 1.96 TeV collected by the CDF experiment. No evidence of a resonance in the diphoton mass spectrum is observed, and upper limits are set on the cross section times branching fraction of the resonant state as a function of Higgs boson mass. The resulting limits exclude Higgs bosons with masses below 106 GeV at a 95% Bayesian credibility level (C.L.) for one fermiophobic benchmark model.

==> HGammaGamma_bib.tex <==
\begin{thebibliography}{41}
\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi
\expandafter\ifx\csname bibnamefont\endcsname\relax
  \def\bibnamefont#1{#1}\fi
\expandafter\ifx\csname bibfnamefont\endcsname\relax
  \def\bibfnamefont#1{#1}\fi
\expandafter\ifx\csname citenamefont\endcsname\relax
  \def\citenamefont#1{#1}\fi
\expandafter\ifx\csname url\endcsname\relax
  \def\url#1{\texttt{#1}}\fi
\expandafter\ifx\csname urlprefix\endcsname\relax\def\urlprefix{URL }\fi
\providecommand{\bibinfo}[2]{#2}
\providecommand{\eprint}[2][]{\url{#2}}

\bibitem[{\citenamefont{Higgs}(1964)}]{Higgs:1964pj}
\bibinfo{author}{\bibfnamefont{P.~W.} \bibnamefont{Higgs}},
  \bibinfo{journal}{Phys. Rev. Lett.} \textbf{\bibinfo{volume}{13}},
  \bibinfo{pages}{508} (\bibinfo{year}{1964}).

\bibitem[{\citenamefont{Djouadi {\it et~al.}.}(1998)\citenamefont{Djouadi, Kalinowski,
  and Spira}}]{Djouadi:1997yw}
\bibinfo{author}{\bibfnamefont{A.}~\bibnamefont{Djouadi}},
  \bibinfo{author}{\bibfnamefont{J.}~\bibnamefont{Kalinowski}},
  \bibnamefont{and} \bibinfo{author}{\bibfnamefont{M.}~\bibnamefont{Spira}},
  \bibinfo{journal}{Comput. Phys. Commun.} \textbf{\bibinfo{volume}{108}},
  \bibinfo{pages}{56} (\bibinfo{year}{1998}).

\bibitem[{\citenamefont{Haber {\it et~al.}.}(1979)\citenamefont{Haber, Kane, and
  Sterling}}]{Haber:1978jt}
\bibinfo{author}{\bibfnamefont{H.~E.} \bibnamefont{Haber}},
  \bibinfo{author}{\bibfnamefont{G.~L.} \bibnamefont{Kane}}, \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{T.}~\bibnamefont{Sterling}},
  \bibinfo{journal}{Nucl. Phys. B} \textbf{\bibinfo{volume}{161}},
  \bibinfo{pages}{493} (\bibinfo{year}{1979}).

\bibitem[{\citenamefont{Gunion {\it et~al.}.}(1990)\citenamefont{Gunion, Vega, and
  Wudka}}]{Gunion:1989ci}
\bibinfo{author}{\bibfnamefont{J.~F.} \bibnamefont{Gunion}},
  \bibinfo{author}{\bibfnamefont{R.}~\bibnamefont{Vega}}, \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{J.}~\bibnamefont{Wudka}},
  \bibinfo{journal}{Phys. Rev. D} \textbf{\bibinfo{volume}{42}},
  \bibinfo{pages}{1673} (\bibinfo{year}{1990}).

\bibitem[{\citenamefont{Basdevant {\it et~al.}.}(1993)}]{Basdevant:1992nb}
\bibinfo{author}{\bibfnamefont{J.~L.} \bibnamefont{Basdevant}}
  \bibnamefont{{\it et~al.}.}, \bibinfo{journal}{Phys. Lett. B}
  \textbf{\bibinfo{volume}{313}}, \bibinfo{pages}{402} (\bibinfo{year}{1993}).

\bibitem[{\citenamefont{Barger {\it et~al.}.}(1992)}]{Barger:1992ty}
\bibinfo{author}{\bibfnamefont{V.}~\bibnamefont{Barger}} \bibnamefont{{\it et~al.}.}
  (\bibinfo{year}{1992}), \eprint{arXiv:hep-ph/9211234}.

\bibitem[{\citenamefont{Akeroyd}(1996)}]{Akeroyd:1995hg}
\bibinfo{author}{\bibfnamefont{A.~G.} \bibnamefont{Akeroyd}},
  \bibinfo{journal}{Phys. Lett. B} \textbf{\bibinfo{volume}{368}},
  \bibinfo{pages}{89} (\bibinfo{year}{1996}).

\bibitem[{\citenamefont{Dobrescu}(2001)}]{Dobrescu:1999gv}
\bibinfo{author}{\bibfnamefont{B.~A.} \bibnamefont{Dobrescu}},
  \bibinfo{journal}{Phys. Rev.} \textbf{\bibinfo{volume}{D63}},
  \bibinfo{pages}{015004} (\bibinfo{year}{2001}).

\bibitem[{\citenamefont{Landsberg and Matchev}(2000)}]{Matchev1}
\bibinfo{author}{\bibfnamefont{G.~L.} \bibnamefont{Landsberg}}
  \bibnamefont{and} \bibinfo{author}{\bibfnamefont{K.~T.}
  \bibnamefont{Matchev}}, \bibinfo{journal}{Phys. Rev. D}
  \textbf{\bibinfo{volume}{62}}, \bibinfo{pages}{035004}
  (\bibinfo{year}{2000}).

\bibitem[{\citenamefont{Mrenna and Wells}(2001)}]{Mrenna}
\bibinfo{author}{\bibfnamefont{S.}~\bibnamefont{Mrenna}} \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{J.~D.} \bibnamefont{Wells}},
  \bibinfo{journal}{Phys. Rev. D} \textbf{\bibinfo{volume}{63}},
  \bibinfo{pages}{015006} (\bibinfo{year}{2001}).

\bibitem[{\citenamefont{Heister {\it et~al.}.}(2002)}]{Heister:2002ub}
\bibinfo{author}{\bibfnamefont{A.}~\bibnamefont{Heister}} \bibnamefont{{\it et~al.}.}
  (\bibinfo{collaboration}{ALEPH Collaboration}), \bibinfo{journal}{Phys. Lett.
  B} \textbf{\bibinfo{volume}{544}}, \bibinfo{pages}{16}
  (\bibinfo{year}{2002}).

\bibitem[{\citenamefont{Abdallah {\it et~al.}.}(2004)}]{Abdallah:2003xf}
\bibinfo{author}{\bibfnamefont{J.}~\bibnamefont{Abdallah}} \bibnamefont{{\it et~al.}.}
  (\bibinfo{collaboration}{DELPHI Collaboration}), \bibinfo{journal}{Eur. Phys.
  J. C} \textbf{\bibinfo{volume}{35}}, \bibinfo{pages}{313}
  (\bibinfo{year}{2004}).

\bibitem[{\citenamefont{Achard {\it et~al.}.}(2003)}]{Achard:2003jb}
\bibinfo{author}{\bibfnamefont{P.}~\bibnamefont{Achard}} \bibnamefont{{\it et~al.}.}
  (\bibinfo{collaboration}{L3 Collaboration}), \bibinfo{journal}{Phys. Lett. B}
  \textbf{\bibinfo{volume}{568}}, \bibinfo{pages}{191} (\bibinfo{year}{2003}).

\bibitem[{\citenamefont{Abbiendi {\it et~al.}.}(2002)}]{Abbiendi:2002yc}
\bibinfo{author}{\bibfnamefont{G.}~\bibnamefont{Abbiendi}} \bibnamefont{{\it et~al.}.}
  (\bibinfo{collaboration}{OPAL Collaboration}), \bibinfo{journal}{Phys. Lett.
  B} \textbf{\bibinfo{volume}{544}}, \bibinfo{pages}{44}
  (\bibinfo{year}{2002}).

\bibitem[{\citenamefont{Rosca}(2002)}]{Rosca:2002me}
\bibinfo{author}{\bibfnamefont{A.}~\bibnamefont{Rosca}}
  (\bibinfo{collaboration}{LEP}) (\bibinfo{year}{2002}),
  \eprint{arXiv:hep-ex/0212038}.

\bibitem[{\citenamefont{Affolder {\it et~al.}.}(2001)}]{Affolder:2001hx}
\bibinfo{author}{\bibfnamefont{A.~A.} \bibnamefont{Affolder}}
  \bibnamefont{{\it et~al.}.} (\bibinfo{collaboration}{CDF Collaboration}),
  \bibinfo{journal}{Phys. Rev. D} \textbf{\bibinfo{volume}{64}},
  \bibinfo{pages}{092002} (\bibinfo{year}{2001}).

\bibitem[{\citenamefont{Abbott {\it et~al.}.}(1999)}]{Abbott:1998vv}
\bibinfo{author}{\bibfnamefont{B.}~\bibnamefont{Abbott}} \bibnamefont{{\it et~al.}.}
  (\bibinfo{collaboration}{D0 Collaboration}), \bibinfo{journal}{Phys. Rev.
  Lett.} \textbf{\bibinfo{volume}{82}}, \bibinfo{pages}{2244}
  (\bibinfo{year}{1999}).

\bibitem[{\citenamefont{Abazov {\it et~al.}.}(2008)}]{hf_D0}
\bibinfo{author}{\bibfnamefont{V.}~\bibnamefont{Abazov}} \bibnamefont{{\it et~al.}.}
  (\bibinfo{collaboration}{D0 Collaboration}), \bibinfo{journal}{Phys. Rev.
  Lett.} \textbf{\bibinfo{volume}{101}}, \bibinfo{pages}{051801}
  (\bibinfo{year}{2008}).

\bibitem[{\citenamefont{Acosta {\it et~al.}.}(2005)}]{Acosta:2004yw}
\bibinfo{author}{\bibfnamefont{D.~E.} \bibnamefont{Acosta}}
  \bibnamefont{{\it et~al.}.} (\bibinfo{collaboration}{CDF Collaboration}),
  \bibinfo{journal}{Phys. Rev. D} \textbf{\bibinfo{volume}{71}},
  \bibinfo{pages}{032001} (\bibinfo{year}{2005}).

\bibitem[{geo()}]{geometry}
\bibinfo{note}{We use a cylindrical coordinate system with its origin in the
  center of the detector, where $\theta$ and $\phi$ are the polar and azimuthal
  angles, respectively, and pseudorapidity is $\eta= - \rm ln$ $\rm
  tan(\theta/2)$. The missing $E_T$ ($\METVEC$) is defined by $\METVEC =
  -\sum_iE_T^i{\hat n}_i, i={\rm calorimeter~tower~number}$, where ${\hat n}_i$
  is a unit vector perpendicular to the beam axis and pointing at the $i^{th}$
  calorimeter tower. $\METVEC$ is corrected for high-energy muons and also jet
  energy corrections. We define $\MET=|\METVEC|$. The transverse momentum $p_T$
  is defined to be $p\sin\theta$.}

\bibitem[{\citenamefont{Sill}(2000)}]{Sill:2000zz}
\bibinfo{author}{\bibfnamefont{A.}~\bibnamefont{Sill}}
  (\bibinfo{collaboration}{CDF Collaboration}), \bibinfo{journal}{Nucl.
  Instrum. Methods} \textbf{\bibinfo{volume}{447}}, \bibinfo{pages}{1}
  (\bibinfo{year}{2000}).

\bibitem[{\citenamefont{Affolder {\it et~al.}.}(2004)}]{Affolder:2003ep}
\bibinfo{author}{\bibfnamefont{A.~A.} \bibnamefont{Affolder}}
  \bibnamefont{{\it et~al.}.} (\bibinfo{collaboration}{CDF Collaboration}),
  \bibinfo{journal}{Nucl. Instrum. Methods} \textbf{\bibinfo{volume}{526}},
  \bibinfo{pages}{249} (\bibinfo{year}{2004}).

\bibitem[{\citenamefont{Balka {\it et~al.}.}(1988)}]{ccal}
\bibinfo{author}{\bibfnamefont{L.}~\bibnamefont{Balka}} \bibnamefont{{\it et~al.}.}
  (\bibinfo{collaboration}{CDF Collaboration}), \bibinfo{journal}{Nucl.
  Instrum. Methods} \textbf{\bibinfo{volume}{267}}, \bibinfo{pages}{272}
  (\bibinfo{year}{1988}).

\bibitem[{\citenamefont{Bertolucci {\it et~al.}.}(1988)}]{wha}
\bibinfo{author}{\bibfnamefont{S.}~\bibnamefont{Bertolucci}}
  \bibnamefont{{\it et~al.}.} (\bibinfo{collaboration}{CDF Collaboration}),
  \bibinfo{journal}{Nucl. Instrum. Methods} \textbf{\bibinfo{volume}{267}},
  \bibinfo{pages}{301} (\bibinfo{year}{1988}).

\bibitem[{\citenamefont{Albrow {\it et~al.}.}(2002)}]{Albrow:2001jw}
\bibinfo{author}{\bibfnamefont{M.~G.} \bibnamefont{Albrow}}
  \bibnamefont{{\it et~al.}.} (\bibinfo{collaboration}{CDF Collaboration}),
  \bibinfo{journal}{Nucl. Instrum. Methods} \textbf{\bibinfo{volume}{480}},
  \bibinfo{pages}{524} (\bibinfo{year}{2002}).

\bibitem[{\citenamefont{Apollinari {\it et~al.}.}(1998)}]{Apollinari:1998bg}
\bibinfo{author}{\bibfnamefont{G.}~\bibnamefont{Apollinari}}
  \bibnamefont{{\it et~al.}.}, \bibinfo{journal}{Nucl. Instrum. Methods}
  \textbf{\bibinfo{volume}{412}}, \bibinfo{pages}{515} (\bibinfo{year}{1998}).

\bibitem[{\citenamefont{Ascoli {\it et~al.}.}(1988)}]{Ascoli:1987av}
\bibinfo{author}{\bibfnamefont{G.}~\bibnamefont{Ascoli}} \bibnamefont{{\it et~al.}.},
  \bibinfo{journal}{Nucl. Instrum. Methods} \textbf{\bibinfo{volume}{268}},
  \bibinfo{pages}{33} (\bibinfo{year}{1988}).

\bibitem[{\citenamefont{Wynne}()}]{Wynne:2009}
\bibinfo{author}{\bibfnamefont{S.}~\bibnamefont{Wynne}}, \bibinfo{note}{{P}h.D.
  thesis, Liverpool University, {F}ERMILAB-THESIS-2007-17}.

\bibitem[{Z_p()}]{Z_pole}
\bibinfo{note}{The CP channel is not used for the 90~\gevcc\ Higgs mass
  hypothesis due to reduced sensitivity caused by contamination from the $Z$
  boson mass peak.}

\bibitem[{\citenamefont{Aaltonen {\it et~al.}.}(2007)}]{RS_PRL}
\bibinfo{author}{\bibfnamefont{T.}~\bibnamefont{Aaltonen}} \bibnamefont{{\it et~al.}.}
  (\bibinfo{collaboration}{CDF Collaboration}), \bibinfo{journal}{Phys. Rev.
  Lett.} \textbf{\bibinfo{volume}{99}}, \bibinfo{pages}{171801}
  (\bibinfo{year}{2007}).

\bibitem[{\citenamefont{Abe {\it et~al.}.}(1993)}]{Abe:1993qb}
\bibinfo{author}{\bibfnamefont{F.}~\bibnamefont{Abe}} \bibnamefont{{\it et~al.}.}
  (\bibinfo{collaboration}{CDF Collaboration}), \bibinfo{journal}{Phys. Rev. D}
  \textbf{\bibinfo{volume}{48}}, \bibinfo{pages}{2998} (\bibinfo{year}{1993}).

\bibitem[{\citenamefont{Sjostrand {\it et~al.}.}(2001)}]{PYTHIA}
\bibinfo{author}{\bibfnamefont{T.}~\bibnamefont{Sjostrand}}
  \bibnamefont{{\it et~al.}.}, \bibinfo{journal}{Comput. Phys. Commun.}
  \textbf{\bibinfo{volume}{135}}, \bibinfo{pages}{238} (\bibinfo{year}{2001}).

\bibitem[{\citenamefont{Brun {\it et~al.}.}(1987)}]{GEANT3}
\bibinfo{author}{\bibfnamefont{R.}~\bibnamefont{Brun}} \bibnamefont{{\it et~al.}.}
  (\bibinfo{year}{1987}), \bibinfo{note}{unpublished, {C}ERN-DD/EE/84-1}.

\bibitem[{\citenamefont{Grindhammer {\it et~al.}.}(1990)\citenamefont{Grindhammer,
  Rudowicz, and Peters}}]{GFLASH}
\bibinfo{author}{\bibfnamefont{G.}~\bibnamefont{Grindhammer}},
  \bibinfo{author}{\bibfnamefont{M.}~\bibnamefont{Rudowicz}}, \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{S.}~\bibnamefont{Peters}},
  \bibinfo{journal}{Nucl. Instrum. Methods} \textbf{\bibinfo{volume}{290}},
  \bibinfo{pages}{469} (\bibinfo{year}{1990}).

\bibitem[{\citenamefont{Lai {\it et~al.}.}(2000)}]{CTEQ5L}
\bibinfo{author}{\bibfnamefont{H.~L.} \bibnamefont{Lai}} \bibnamefont{{\it et~al.}.}
  (\bibinfo{collaboration}{CTEQ Collaboration}), \bibinfo{journal}{Eur. Phys.
  J.} \textbf{\bibinfo{volume}{C12}}, \bibinfo{pages}{375}
  (\bibinfo{year}{2000}).

\bibitem[{\citenamefont{Field and Group}(2005)}]{TUNEA}
\bibinfo{author}{\bibfnamefont{R.}~\bibnamefont{Field}} \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{R.~C.} \bibnamefont{Group}}
  (\bibinfo{collaboration}{CDF Collaboration}) (\bibinfo{year}{2005}),
  \eprint{ArXiv:hep-ph/0510198}.

\bibitem[{ISR()}]{ISR}
\bibinfo{note}{We constrain the rate of initial state radiation using Drell-Yan
  events in data.}

\bibitem[{\citenamefont{Mrenna and Yuan}(1998)}]{MrennaQCD}
\bibinfo{author}{\bibfnamefont{S.}~\bibnamefont{Mrenna}} \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{C.~P.} \bibnamefont{Yuan}},
  \bibinfo{journal}{Phys. Lett. B} \textbf{\bibinfo{volume}{416}},
  \bibinfo{pages}{200} (\bibinfo{year}{1998}).

\bibitem[{\citenamefont{Stump {\it et~al.}.}(2003)}]{CTEQ6.1M}
\bibinfo{author}{\bibfnamefont{D.}~\bibnamefont{Stump}} \bibnamefont{{\it et~al.}.},
  \bibinfo{journal}{J. High Energy Phys.} \textbf{\bibinfo{volume}{0410}},
  \bibinfo{pages}{046} (\bibinfo{year}{2003}).

\bibitem[{\citenamefont{Bourilkov {\it et~al.}.}(2006)\citenamefont{Bourilkov, Group,
  and Whalley}}]{Weights}
\bibinfo{author}{\bibfnamefont{D.}~\bibnamefont{Bourilkov}},
  \bibinfo{author}{\bibfnamefont{R.~C.} \bibnamefont{Group}}, \bibnamefont{and}
  \bibinfo{author}{\bibfnamefont{M.~R.} \bibnamefont{Whalley}}
  (\bibinfo{year}{2006}), \eprint{arXiv:hep-ph/0605240}.

\bibitem[{\citenamefont{Amsler {\it et~al.}.}(2008)}]{Amsler:2008zz}
\bibinfo{author}{\bibfnamefont{C.}~\bibnamefont{Amsler}} \bibnamefont{{\it et~al.}.}
  (\bibinfo{collaboration}{Particle Data Group}), \bibinfo{journal}{Phys. Lett.
  B} \textbf{\bibinfo{volume}{667}}, \bibinfo{pages}{1} (\bibinfo{year}{2008}).

\end{thebibliography}

